Tree Space Prototypes: Another Look at Making Tree Ensembles Interpretable

Ensembles of decision trees perform well on many problems, but are not interpretable. In contrast to existing approaches in interpretability that focus on explaining relationships between features and predictions, we propose an alternative approach to interpret tree ensemble classifiers by surfacing representative points for each class -- prototypes. We introduce a new distance for Gradient Boosted Tree models, and propose new, adaptive prototype selection methods with theoretical guarantees, with the flexibility to choose a different number of prototypes in each class. We demonstrate our methods on random forests and gradient boosted trees, showing that the prototypes can perform as well as or even better than the original tree ensemble when used as a nearest-prototype classifier. In a user study, humans were better at predicting the output of a tree ensemble classifier when using prototypes than when using Shapley values, a popular feature attribution method. Hence, prototypes present a viable alternative to feature-based explanations for tree ensembles.

==> tables/imbalance_stats.tex <==
\begin{table}
\centering
\begin{tabular}{lllllll}
\toprule
& & & \multicolumn{4}{c}{$k$, number of prototypes} \\
\cmidrule{4-7}
Dataset & Model & Method  &  4 & 8 & 16 & 32  \\
\midrule

\multirow{4}{*}{Breastcancer} & \multirow{2}{*}{RF}  &  SM-A & 2,2 & 3,5 & 7,9 & 13,19\\
 & & SG &  2,2 & 2,2 & 2,2 & 2,2\\
\cmidrule{2-7}
 & \multirow{2}{*}{GB}  &  SM-A & 2,2 & 4,4 & 6,10 & 14,18\\
 & & SG & 2,2 & 2,3 & 2,3 & 2,3\\
\midrule
\multirow{4}{*}{Diabetes} & \multirow{2}{*}{RF}  &  SM-A & 2,2 & 5,3 & 10,6 & 19,13\\
 & & SG & 2,2 & 4,4 & 7,5 & 7,5\\
\cmidrule{2-7}
 & \multirow{2}{*}{GB}  &  SM-A & 2,2 & 5,3 & 10,6 & 21,11\\
 & & SG & 3,1 & 5,3 & 11,5 & 16,11\\
\midrule
\multirow{4}{*}{T-COMPAS} & \multirow{2}{*}{RF}  &  SM-A & 1,3 & 2,6 & 4,12 & 10,22\\
 & & SG & 2,2 & 3,5 & 6,10 & 9,13\\
\cmidrule{2-7}
 & \multirow{2}{*}{GB}  &  SM-A & 1,3 & 2,6 & 7,9 & 13,19\\
 & & SG &  2,2 & 2,5 & 2,5 & 2,5\\
\midrule
\multirow{4}{*}{RHC} & \multirow{2}{*}{RF}  &  SM-A &  3,1 & 5,3 & 11,5 & 19,13\\
 & & SG &  2,2 & 4,4 & 8,8 & 15,17\\
\cmidrule{2-7}
 & \multirow{2}{*}{GB}  &  SM-A &  2,2 & 5,3 & 9,7 & 18,14\\
 & & SG &  2,2 & 5,3 & 11,5 & 21,11\\
\midrule
%\multirow{6}{*}{MNIST} & \multirow{2}{*}{Mahalanobis}  &  SM-all & \\
% & & Greedy-accuracy & \\
%\cmidrule{2-8}
%\multirow{4}{*}{MNIST 3-5} & \multirow{2}{*}{RF}  &  SM-all & \\
%& & Greedy-accuracy & \\
%\cmidrule{2-8}
%& \multirow{2}{*}{GB $vg^2$}  &  SM-all & \\
%& & Greedy-accuracy & \\
%\midrule
\end{tabular}
\caption{Number of prototypes found for each class across different datasets. The first number represents the number of class 0 prototypes, the second number represents the number of class 1 prototypes. The dataset label imbalances are as follows: 35\% of observations in Diabetes had label 1; 63\% for breast cancer, 69\% for Turker-COMPAS, 38\% for RHC.}
\label{tab:imbalance_stats}
\end{table}
% MNIST dataset statistics: https://git-disl.github.io/GTDLBench/datasets/mnist_datasets/

%53\% for MNIST. \note{MNIST number to be confirmed}

==> tables/proximity_stats.tex <==
\begin{table*}
\centering
\begin{tabular}{llllllllll}
\toprule
& &  \multicolumn{3}{c}{RF Distance Percentiles}  & \multicolumn{3}{c}{GB Distance Percentiles}\\
\cmidrule(r){3-5} \cmidrule(l){6-8}
Dataset  & Observations &  5 & 50 & 95  &  5 & 50 & 95 \\
\midrule
\multirow{3}{*}{Breastcancer} & All &  0.030 & 0.840 & 1.000 & 0.000 & 0.530 & 1.000\\
 &  Same class &  0.020 & 0.280 & 0.940  & 0.000 & 0.130 & 0.700\\
   & Different class  &  0.870 & 1.000 & 1.000   & 0.540 & 1.000 & 1.000\\
\midrule
\multirow{3}{*}{Diabetes} & All  &  0.670 & 0.990 & 1.000 & 0.290 & 0.740 & 0.980\\
 &  Same class  &  0.560 & 0.970 & 1.000  & 0.240 & 0.690 & 0.940\\
   & Different class  &  0.830 & 0.990 & 1.000   & 0.380 & 0.800 & 0.980\\
\midrule
\multirow{3}{*}{T-COMPAS} & All  &  0.750 & 1.000 & 1.000 & 0.090 & 0.840 & 1.000\\
 &  Same class  &  0.710 & 1.000 & 1.000  & 0.070 & 0.840 & 1.000\\
   & Different class  &  0.820 & 1.000 & 1.000   & 0.120 & 0.850 & 1.000\\
\midrule
\multirow{3}{*}{RHC} & All  &  0.950 & 1.000 & 1.000 & 0.420 & 0.610 & 0.750\\
 &  Same class  &  0.930 & 1.000 & 1.000  & 0.410 & 0.600 & 0.750\\
   & Different class  &  0.970 & 1.000 & 1.000   & 0.440 & 0.620 & 0.750\\
\midrule
\multirow{3}{*}{MNIST 3-5} & All  &  0.150 & 1.000 & 1.000 & 0.340 & 0.880 & 1.000\\
 &  Same class  &  0.050 & 0.820 & 1.000  & 0.250 & 0.690 & 0.980\\
   & Different class  &  0.990 & 1.000 & 1.000   & 0.760 & 0.960 & 1.000\\
\midrule
\bottomrule
\end{tabular}
\caption{Statistics of RF and GBT distances ($1 - \text{proximity}$) on different datasets. }
\label{tab:proximit_stats}
\end{table*}
